Resonant Floquet Scattering of Ultracold Atoms

In systems of ultracold atoms, pairwise interactions are resonantly enhanced by the application of an oscillating magnetic field that is parallel to the spin-quantization axis of the atoms. The resonance occurs when the frequency of the applied field is precisely tuned near the transition frequency between the scattering atoms and a diatomic molecule. The resulting cross section can be made more than two orders of magnitude larger than the cross section in the absence of the oscillating field. The low momentum resonance properties have a universal description that is independent of the atomic species. To arrive at these conclusions, we first develop a formal extension of Floquet theory to describe scattering of atoms with time-periodic, short-range interaction potentials. We then calculate the atomic scattering properties by modeling the atomic interactions with a square well potential with oscillating depth and then explicitly solving the time-dependent Schrodinger equation. We then apply the Floquet formalism to the case of atoms scattering with a contact interaction described by a time-periodic scattering length, obtaining analytic results that agree with those obtained by solving the time-dependent Schrodinger equation.

==> Misc/acronyms.tex <==
% !TEX root = WendtPhDThesis.tex
\newacronym{ANC}{ANC}{Asymptotic Normalization Coefficient}
\newacronym{COM}{COM}{center-of-mass}

\newacronym{NN}{NN}{nucleon-nucleon}
\newacronym{2NF}{2NF}{two-nucleon force}
\newacronym{3NF}{3NF}{three-nucleon force}
\newacronym{AV18}{AV18}{Argonne $v_{18}$}

\newacronym{QCD}{QCD}{Quantum Chromodynamics}
\newacronym{QED}{QED}{Quantum Electrodynamics}
\newacronym{QFT}{QFT}{Quantum Field Theory}

\newacronym{SVD}{SVD}{singular value decomposition}


\newacronym{EFT}{EFT}{effective field theory}
\newacronym{RG}{RG}{renormalization group}
\newacronym{SRG}{SRG}{Similarity Renormalization Group}

\newacronym{SVM}{SVM}{stochastic variational method}

\newacronym{HO}{HO}{Harmonic Oscillator}

\newacronym{HF}{HF}{Hartree-Fock}
\newacronym{HFB}{HFB}{Hartree-Fock-Bogoliubov}

\newacronym{QMC}{QMC}{Quantum Monte Carlo}
\newacronym{CC}{CC}{Coupled Cluster}
\newacronym{NCSM}{NCSM}{No Core Shell Model}
\newacronym{itNCSM}{IT-NCSM}{Importance Truncated No Core Shell Model}
\newacronym{ShM}{SM}{Shell Model}
\newacronym{DFT}{DFT}{density functional theory}
\newacronym{VMC}{VMC}{variational Monte Carlo}
\newacronym{GFMC}{GFMC}{Green's function Monte Carlo}
\newacronym{AFDMC}{AFDMC}{Auxiliary Field Diffusion Monte Carlo}
\newacronym{MFD}{MFD}{many fermion dynamics}
\newacronym{CI}{CI}{configuration interaction}
\newacronym{NCFC}{NCFC}{No Core Full Configuration}
\newacronym{FCI}{FCI}{Full Configuration Interaction}
\newacronym{MBPT}{MBPT}{many-body perturbation theory}


\newacronym{UV}{UV}{ultraviolet}
\newacronym{IR}{IR}{infrared}

\newacronym{NUCLEI}{NUCLEI}{NUclear Computational Low-Energy Initiative}
\newacronym{UNEDF}{UNEDF}{Universal Nuclear Energy Density Functional}

\newacronym{ChPT}{$\chi$-PT}{Chiral Perturbation Theory}
\newacronym{ChEFT}{$\chi$-EFT}{Chiral Effective Field Theory}

\newacronym{DCT}{DCT}{Discrete Cosine Transform}

\newacronym{DWBS}{DWBS}{Distorted Wave Born Series}
\newacronym{DWBA}{DWBA}{Distorted Wave Born Approximation}
\newacronym[longplural=ordinary differential equations]{ODE}{ODE}{ordinary differential equation}




==> Misc/lengths.tex <==
% !TEX root = WendtPhDThesis.tex
\newlength{\movieplotwidth}
\setlength{\movieplotwidth}{.98\textwidth}
\newlength{\phaseplotwidth}
\setlength{\phaseplotwidth}{0.29\textwidth}
\newlength{\universalityplotwidth}
\setlength{\universalityplotwidth}{0.9\textwidth}
\newlength{\wideplotwidth}
\newlength{\plotwidth}
\newlength{\plotsep}
\newlength{\mpagewidth}



==> Misc/units.tex <==
% !TEX root = WendtPhDThesis.tex
\newcommand{\fm}{\,\text{fm}}
\newcommand{\km}{\,\text{km}}
\newcommand{\fmi}{\,\text{fm}^{-1}}
\newcommand{\MeV}{\,\text{MeV}}
\newcommand{\GeV}{\,\text{GeV}}
\newcommand{\mev}{\,\text{MeV}}
\newcommand{\keV}{\,\text{keV}}
\newcommand{\eV}{\,\text{eV}}

